DeepFM: An End-to-End Wide & Deep Learning Framework for CTR Prediction

Learning sophisticated feature interactions behind user behaviors is critical in maximizing CTR for recommender systems. Despite great progress, existing methods have a strong bias towards low- or high-order interactions, or rely on expertise feature engineering. In this paper, we show that it is possible to derive an end-to-end learning model that emphasizes both low- and high-order feature interactions. The proposed framework, DeepFM, combines the power of factorization machines for recommendation and deep learning for feature learning in a new neural network architecture. Compared to the latest Wide & Deep model from Google, DeepFM has a shared raw feature input to both its "wide" and "deep" components, with no need of feature engineering besides raw features. DeepFM, as a general learning framework, can incorporate various network architectures in its deep component. In this paper, we study two instances of DeepFM where its "deep" component is DNN and PNN respectively, for which we denote as DeepFM-D and DeepFM-P. Comprehensive experiments are conducted to demonstrate the effectiveness of DeepFM-D and DeepFM-P over the existing models for CTR prediction, on both benchmark data and commercial data. We conduct online A/B test in Huawei App Market, which reveals that DeepFM-D leads to more than 10% improvement of click-through rate in the production environment, compared to a well-engineered LR model. We also covered related practice in deploying our framework in Huawei App Market.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> practical.tex <==
\section{Practical Issues}\label{section:practical}

Due to the fact that we are using this model along with our implementation in our commercial recommender system, it is hardly possible for us to release our code. To help reproduce our models, some implementation details are presented in this section (as shown in Figure~\ref{fig:framework}), such as data processing (in Section~\ref{subsection:data_processing}), model implementation (in Section~\ref{subsection:model_implement}) and two acceleration techniques (in Section~\ref{subsection:Accelerating}). Moreover, extensive experiments are conducted to validate the effectiveness of such techniques.

\subsection{Data Processing}\label{subsection:data_processing}

\begin{figure*}[ht]
\centering
\includegraphics[width=0.95\textwidth]{img/Framework.pdf}
\caption{The details of of DeepFM framework, including data processing, model implementation, and accelerating strategies.}\label{fig:framework}
\end{figure*}

%\begin{figure}[ht]
%\centering
%\includegraphics[width=0.45\textwidth]{img/DataProcessing.pdf}
%\caption{Data Processing.}\label{fig:DataProcess}
%\end{figure}


\subsubsection{Input Construction}

The general steps of data processing are displayed in the left upper part of Figure~\ref{fig:framework}. Firstly, we pass through the entire \emph{raw input data} to get the statistics of each field (e.g., the number of unique features in each categorical field, the max/min/avg value of each numerical fields) and also construct a local identifier for each feature within each field. Then, the global identifier (we refer it as \emph{ID input data}) of the $\rm j^{th}$ feature in $\rm i^{th}$ field can be computed as ${\rm GlobalID}({\rm i,j}) = \sum_{\rm k=1}^{\rm i-1}{n_{\rm k}}+{\rm j}$, where ${\rm i\geq 1}$, ${\rm j}$ starts from zero, and $n_{\rm k}$ is the number of features of ${\rm k^{th}}$ field.
%For example, the global identifier of feature ``Location: Hong Kong" is: \[{\rm GlobalID}(2,1) = \sum_{\rm k=1}^{\rm 1}{n_{\rm k}} + {\rm j} = n_{\rm 1} + {\rm j} = 2 + 1 = 3.\]
There are two methods to deal with numerical fields. The first method is discretizing the numerical value.
%For instance, feature value ``Age: 39" becomes ``Age: 3" if the age value is discretized by taking the floor after being divided by ten.
The other option is retaining the numerical value as it is. With this approach, all the features of this numerical field share the same global identifier and they are distinguished by the feature value.
%For instance ``Age: 39" and ``Age: 60" are encoded as ``$10: 39$" and ``$10: 60$", under the assumption that the global identifier of ``Age" field is 10.
%By now, we cover the case of handling categorical fields. Normally, there are two different methods to deal with numerical fields. The first direction goes to discretize the numerical values. For instance, feature value ``Age: 39" becomes ``Age: 3" if the age value is discretized by taking the floor after dividing by ten. The other option is retain the numerical value as it is. With this approach, all the features of this numerical field share the same global identifier and they are distinguished by the feature value. For instance ``Age: 39" and ``Age: 60" are encoded as ``$10: 39$" and ``$10: 60$", under the assumption that the global identifier of ``Age" field is 10.
%The general steps of data processing are displayed in the left upper part of Figure~\ref{fig:framework}. To make readers understand the procedure of data processing better, we give a running example in Figure~\ref{fig:DataProcess}. As we can see, the original data set consists of raw features (we refer it as \emph{raw input data}). For instance in step 1 of Figure~\ref{fig:DataProcess}, the first data record in our example is (Gender: Male, Location: Shenzhen, Item Type: Game, click: 1). For now, we consider only categorical fields, such as gender, location, item type in our example, while we will discuss the case of numerical fields later. \emph{One-hot encoding} is widely used to encode categorical fields, which assigns a global identifier to each feature, as shown in step 3 of Figure~\ref{fig:DataProcess} (we refer it as \emph{ID input data}). Note that we follow the input data format of libSVM \cite{LibSVM}. Before generating a global identifier for each feature, as shown in step 2 of Figure~\ref{fig:DataProcess}, we pass through the entire data set to get the statistics of each field (e.g., the number of unique features in each categorical field, the max/min/avg value of each numerical fields). Meanwhile in step 2, we also construct a local identifier for each feature within each field. For instance, in field ``Gender", the number of feature is 2, and the local identifier for each feature is ``Male:0" and ``Female:1". Given the local identifier $j$ of a feature of $i^{th}$ field, its global identifier can be computed as \[GlobalID(i,j) = \sum_{k=1}^{k=i-1}{n_k}+j\] where $i\geq 1$, $j$ starts from zero, and $n_k$ is the number of unique features of $k^{th}$ field. Let us compute the global identifier of feature value ``Location: Hong Kong" as an example: \[GlobalID(2,1) = \sum_{k=1}^{k=1}{n_k} + j = n_1 + j = 2 + 1 = 3\]
\subsubsection{Online mapping V.S. Offline indexing}

%Whether storing \emph{ID input data}, is an option.
There are two possibilities that we implement: \emph{online mapping} and \emph{offline indexing}. Online mapping does not store ID input data physically and does the transformations from local identifiers to global identifiers every time reading raw input data. On the contrary, with additional storage, offline indexing stores ID input data so that we can read it directly without doing the transformations every time. Therefore, if one's algorithm needs to read the data one or very few times, Online mapping is sufficient. While offline indexing is better when multiple epoches of data reading is necessary. Since DeepFM models need to pass tens of epoches of data to be trained well, we choose to adopt offline indexing.

%Every coin has two sides. \emph{offline indexing} needs extra storage costs and efficiency cost to store ID input data. Therefore, if one's algorithm needs to read the data one or very few times, it is enough to choose \emph{Online mapping}. On the other side, if multiple epoches of data reading is necessary, \emph{offline indexing} is a better option. In our case, DeepFM models need to pass tens of epoches of data to be trained well. Therefore, we choose to adopt \emph{offline indexing}, which initially sacrifices storage and running time efficiency to store ID input data, but benefits from avoiding transformation from local identifiers to global identifiers for each feature value.



%Generally, the deep model need to be trained several epoches, where one epoch means training the data set one round. However, through our statistical analysis, feature mapping online takes a large percentage of training time (\textcolor{red}{concrete number}). So it is time consuming if we conduct feature mapping online repeatedly in every epoch. For the purpose of improving training efficiency, we deploy offline index strategy in our framework. Specifically, we do feature mapping once and save these model-readable vectors as offline index. Therefore, the proportion of training time in data processing is reduced, and as a result, the training process is able to be more efficiency.

\subsection{Model Implementation Details}\label{subsection:model_implement}
In this section, we present the details of our implementation\footnote{All the compared models are implemented with Tensorflow \cite{tensorflow}.}, including model implementation and layer normalization, of DeepFM (as shown in the right upper part of Figure~\ref{fig:framework}). Note that the pseudo code of DeepFM models are presented in a Tensorflow-style. Moreover, for the clarity, some Tensorflow functions are summarized in Table~\ref{table:tffunction}.

\begin{table}
\centering
\small
\caption{\small{The abbreviation of Tensorflow function.}}\label{table:tffunction}
\begin{tabular}{|c|c|}
\hline
Abbreviation & Tensorflow Function  \\ \hline
Opt & tf.train.AdamOptimizer  \\ \hline
Logloss & tf.nn.sigmoid\_cross\_entropy\_with\_logits\\ \hline
NN & PNN or DNN \\ \hline
\multirow{2}{*}{tf\_X} & tf.placeholder(tf.int32, shape=[None, m]), \\
&\emph{input features} \\ \hline
tf\_Y & tf.placeholder(tf.int32), \emph{output labels}\\ \hline
\end{tabular}
\end{table}
\subsubsection{Model Implementation}
The details of DeepFM model implementation are presented in the following. In line 2, the parameters \texttt{w} and \texttt{V} are initialized. Then Line 3 to line 6 compute several meta parameters for calculating prediction from FM component. FM and deep predictions are computed in line 7 and line 8 respectively. Finally, the \texttt{logits} of our model are computed by the summation of predictions from FM and deep component. The \texttt{loss} between the logits and the labels is computed in line 11, and the model parameters are trained by back-propagating the gradients in line 12.
%Note that in line 12 we take the Adam optimizer as an example, but other optimizers are also possible by calling different functions.
%Due to the fact that we are using DeepFM along with our implementation in our commercial recommender system, our code will not be released. In order to help people implement our models easily,

\begin{lstlisting}[frame=tb]{somecode}
def DeepFM(hyper_parameter):
  self.w,self.V = initial(hyper_parameter);
  wx = tf.gather(self.w, tf_X);
  vx = tf.gather(self.V, tf_X);
  vx2 = tf.square(tf.reduce_sum(vx, 1));
  vxs = tf.reduce_sum(tf.square(vx), 1);
  FM = 0.5*tf.reduce_sum(vx2 - vxs, 1) + tf.reduce_sum(wx, 1);
  Deep = NN(hyper_parameter, vx);
  logits = FM + Deep
  pred = tf.sigmoid(logits, tf_Y);
  loss = Logloss(logits, Y);
  appGrad = Opt.minimize(loss);
\end{lstlisting}



%In the \texttt{test mode} (line 12 to line 14), we make the prediction (line 14) given the feature values of a data record, after computing the logits in line 13.
%
%The details of \texttt{forward} function are displayed in line 15 to line 22. Predictions from FM component and Deep component are computed in line 20 and line 21, respectively. Line 16 to line 19 compute several meta parameters for calculating prediction from FM component. Finally, \texttt{forward} function returns summation of predictions from FM component and Deep component as the logits of our model. Note that in line 21, the prediction from Deep component differs from each other as the neural network structure is different, in particular, the \texttt{NN} function needs to implement according to a given neural network structure. For instance, DeepFM-IP, DeepFM-OP, DeepFM-P$\ast$ and DeepFM-D need to implement different \texttt{NN} functions in line 21.

\subsubsection{Layer Normalization}

Layer normalization~\cite{LN} is a technique which normalizes the activities of the neurons to reduce the training time. Layer normalization computes the mean and variance for normalization from all the summed inputs to the neurons in a certain layer on a training record. The implementation pseudo code is presented below. Mean (\texttt{m}) and variance (\texttt{var}) of the summed inputs of all the neurons in a certain layer are computed in line 14. As in line 15, the summed input of each neuron is normalized by the computed mean and variance value, where epsilon (\texttt{ep}) is a user-defined constant. Finally, the normalized values are linearly scaled by two parameters \texttt{gain} and \texttt{bias}, which are trainable during the learning process, as presented in line 16.
%To achieve this goal, batch normalization~\cite{BN} computes the mean and variance of the summed input to a neuron over a mini-batch of training records which are then used to normalize the summed input to that neuron on each training record.

\begin{lstlisting}[frame=tb]{somecode}
def LN(in, gain, bias, ep):
  m,var=tf.nn.moments(in,[1],keep_dims=True)
  LN_in=(in - m)/tf.sqrt(var + ep)
  return LN_in * gain + bias
\end{lstlisting}

\begin{figure}[ht]
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{-10pt}
\centering
\begin{minipage}[b]{0.5\textwidth}\centering
\includegraphics[width=0.48\textwidth]{img/LN_1GPU_AUC.png}
\includegraphics[width=0.48\textwidth]{img/LN_1GPU_LOSS.png}
\end{minipage}
\caption{\small{performance comparison of DeepFM-D w/o layer normalization.}}\label{fig:LN}
\end{figure}

We evaluate the effectiveness of layer normalization in our DeepFM-D model on Company$\ast$ data set. Figure~\ref{fig:LN} presents the test curves of AUC and Logloss where $x$-axis is the number of epoch. As shown in Figure~\ref{fig:LN}, the AUC and Logloss are almost the same w/o layer normalization at the $10^{th}$ epoch, however the DeepFM-D model with layer normalization is convergent faster than the case without layer normalization. We also evaluate the efficiency of layer normalization and we observe that deploying layer normalization in each hidden layers (in our case there are three hidden layers) of DeepFM-D introduces 4\% cost in terms of running time.

\subsection{Accelerating}\label{subsection:Accelerating}

\subsubsection{Multi-GPU Architecture}

In this section, we present our first accelerating technique, namely multi-GPU data parallelism. The pseudo code is presented below\footnote{Because the parameter definitions and initialization operations are similar with Section~\ref{subsection:model_implement}, we omit these replicate items.}. Since we adopt data parallelism, a batch of data records is split into \texttt{Num\_GPU} pieces, where \texttt{NUM\_GPU} is the number of GPU cards (line 18 to line 19). The basic idea (which is shown in the right lower part of Figure~\ref{fig:framework}) is that the gradients of different pieces of data records are computed and averaged, then the model parameters are updated by the averaged gradients. Arrays to store global gradients and losses over multi-GPUs are defined in line 20. Each GPU does the same operations as in line 22 to line 27. The \texttt{logits} of the data records distributed on this GPU are computed in the same way as \emph{DeepFM function} in line 23, the \texttt{loss} are computed by \texttt{Logloss} in line 24.
%Line 25 refines the variable scope to share the same variables defined in this model.
The gradients (\texttt{grads}) are computed in line 25. As in line 26 to line 27, gradients  and losses are stored in the arrays defined previously. Lastly, the average gradients are computed in line 28 and the model parameters are updated accordingly in line 29.

\begin{lstlisting}[frame=tb]{somecode}
def MGPUDeepFM(NUM_GPU, others are same as DeepFM):
  X_S = tf.split(0, NUM_GPU, tf_X);
  Y_S = tf.split(0, NUM_GPU, tf_Y);
  gtGrads = []; gtLoss = [];
  for i in xrange(NUM_GPU):
    with tf.device('/gpu:%d' % i):
    logits = FM(X_S[i]) + Deep(X_S[i]);
    loss = Logloss(logits, Y_S[i]);
    grads = Opt.compute_gradients(loss);
    gtGrads.append(grads);
    gtLoss.append(loss);
  avgGrad = average_gradients(gtGrads);
  appGrad = Opt.apply_gradients(avgGrad);
\end{lstlisting}

We evaluate the effectiveness of multi-GPU data parallelism of DeepFM-D model on Company$\ast$ data set, in terms of AUC and Logloss. In our experiments, we equip with 4 Nvidia Tesla K40 GPU cards. Figure~\ref{fig:multi-cards} presents the test curves of AUC and Logloss comparison of using multiple GPU cards and using a single GPU core. With 4 GPU cards, AUC and Logloss decrease 0.14\% and 0.52\%, respectively, compared to using a single GPU card.

\begin{figure}[ht]
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{-10pt}
\centering
\begin{minipage}[b]{0.5\textwidth}\centering
\includegraphics[width=0.48\textwidth]{img/multiGPU_AUC.png}
\includegraphics[width=0.48\textwidth]{img/multiGPU_LOSS.png}
\end{minipage}
\caption{\small{performance comparison of multiple GPU data parallelism of DeepFM-D model.}}\label{fig:multi-cards}
\end{figure}



\subsubsection{Asynchronous Data Reading}

Training a neural network is usually in a mini-batch style, in which a mini-batch of data records (e.g., several thousand) is read and fed into the neural network, and then model parameters are updated in a forward-backward way. There are two possible ways to handle data reading and model updating: sequential and parallel, as shown in the left lower part of Figure~\ref{fig:framework}. In the sequential approach, data reading and model updating are processed interleaved and sequentially, i.e., model updating starts when the current mini-batch of data is read and fed, and the next mini-batch of data will not be read until the model finishes updating with the current mini-batch of data. Obviously, this is not an efficient way. We propose a parallel manner to handle data reading and model updating, namely, \emph{asynchronous data reading}. A thread is created to read the data records regardless of the model updating, so that the model parameters keep updating without interrupted by reading data.

The pseudo-code of asynchronous data reading is presented as below. A first-in-first-out queue is defined in line 30. Two actions, namely enqueue and dequeque, are defined in line 31 and line 32, respectively. Line 33 to line 39 define the enqueue operation in detail, where \texttt{sess} is a object defined by \texttt{tf.Session()}. For each GPU card in multi-GPU setting, data records keep being read and enqueued. A thread is created in line 40 to run the \texttt{eq()} function. The created thread starts to work as in line 41 to line 42. In line 43, once started by \texttt{tf.train.start\_queue\_runners}\cite{TensorflowQueueRunner}, the QueueRunner will launch the threads in the back-end to fill the queue. Meanwhile the main thread will execute the dequeue operation to pull data from the \texttt{FIFOQueue}.

\begin{lstlisting}[frame=tb]{somecode}
FQ=tf.FIFOQueue
EqOp=FQ.enqueue([X,Y]);
X_q,Y_q=FQ.dequeue();
def eq(sess):
  while True:
  X=[]; Y=[];
  for _gpu in range(NUM_GPU):
    X_S,Y_S=train_gen.next();
    X.extend(X); Y.extend(Y);
    sess.run(EqOp,feed_dict={X:X,Y:Y});
EqTh=threading.Thread(target=eq,args=[sess])
EqTh.isDaemon();
EqTh.start();
Th=tf.train.start_queue_runners(sess=sess);
\end{lstlisting}


\subsection{Efficiency Validation Experiment}\label{subsection:Validation}

As shown in Table~\ref{table:valiadtion}, we record the speed up rate\footnote{In this paper, we define the speed up rate of strategy A over strategy B to be the processing time of strategy B divided by the process time of strategy A.} of offline indexing (OI) over online mapping (OM) , the 4-GPU over 1-GPU data parallelism, asynchronous (Asyn) over synchronous (Syn) data reading of DeepFM models on Company$\ast$ and Criteo data sets. In addition, compared with the basic version (OM, 1-GPU and Syn), the efficiency is improved by more than 1300\% and 600\% on Company$\ast$ and Criteo-Random data sets when applying OI, 4-GPU and Syn techniques. We omit the validation result on Criteo-Sequential data set, since Criteo-Sequential and Criteo-Random come from the same original data set with different splitting strategies.
\begin{table}[ht]
\centering
\small
\caption{\small{Speed up rate for DeepFM-D model.}}\label{table:valiadtion}
\begin{tabular}{|c|c|c|}
\hline
                   & Company$\ast$ & Criteo-Random \\ \hline
 OI over OM    & 5.25 X          & 2.57 X   \\ \hline
 4-GPU over 1-GPU    & 2.25 X          & 2.15 X   \\ \hline
 Asyn over Syn     & 1.12 X          & 1.19 X  \\ \hline
 {Asyn + 4-GPU + OI over}      &   \multirow{2}{*}{13.12 X}        & \multirow{2}{*}{6.42 X}  \\
 Syn + 1-GPU + OM & &\\ \hline
\end{tabular}
\end{table}

